Optimizing Design and Control Methods for Using Collaborative Robots in Upper-Limb Rehabilitation

In this paper, we address the development of a robotic rehabilitation system for the upper limbs based on collaborative end-effector solutions. The use of commercial collaborative robots offers significant advantages for this task, as they are optimized from an engineering perspective and ensure safe physical interaction with humans. However, they also come with noticeable drawbacks, such as the limited range of sizes available on the market and the standard control modes, which are primarily oriented towards industrial or service applications. To address these limitations, we propose an optimization-based design method to fully exploit the capability of the cobot in performing rehabilitation tasks. Additionally, we introduce a novel control architecture based on an admittance-type Virtual Fixture method, which constrains the motion of the robot along a prescribed path. This approach allows for an intuitive definition of the task to be performed via Programming by Demonstration and enables the system to operate both passively and actively. In passive mode, the system supports the patient during task execution with additional force, while in active mode, it opposes the motion with a braking force. Experimental results demonstrate the effectiveness of the proposed method.

==> trjfilter2.tex <==
%\def\dy{\dot y}
%\def\ddy{\ddot y}
%\def\um{\dddot x_{\mbox{\tiny{m}}}}
%\def\uM{\dddot x_{\mbox{\tiny{M}}}}
%\def\dym{\dot y_{\mbox{\tiny{m}}}}
%\def\dyM{\dot y_{\mbox{\tiny{M}}}}
%\def\ddym{\ddot y_{\mbox{\tiny{m}}}}
%\def\ddyM{\ddot y_{\mbox{\tiny{M}}}}
%\def\umM{(\um-\uM)}
%%\def\umM{\ddot x_{\mbox{\tiny{mM}}}}
%\def\D{(\ddy^2 - 2\dy\uM)}

\def\dy{\dot y}
\def\ddy{\ddot y}
%\def\dddxm{\jerk_{\mbox{\tiny{m}}}}
%\def\um{\dddxm}
%\def\dddxM{\jerk_{\mbox{\tiny{M}}}}
%\def\uM{\dddxM}
%\def\ddxm{\acc_{\mbox{\tiny{m}}}}
%\def\ddxM{\acc_{\mbox{\tiny{M}}}}
%\def\dxm{\vel_{\mbox{\tiny{m}}}}
%\def\dxM{\vel_{\mbox{\tiny{M}}}}
%\def\dym{\dot y_{\mbox{\tiny{m}}}}
%\def\dyM{\dot y_{\mbox{\tiny{M}}}}
%\def\ddym{\ddot y_{\mbox{\tiny{m}}}}
%\def\ddyM{\ddot y_{\mbox{\tiny{M}}}}


\newcommand{\xM}[1]{\overline{x}_{#1}}
\newcommand{\xm}[1]{\underline{x}_{#1}}

\newcommand{\yM}[1]{\overline{y}_{#1}}
\newcommand{\ym}[1]{\underline{y}_{#1}}

\def\dddxm{\xm{0}}
\def\um{\dddxm}
\def\dddxM{\xM{0}}
\def\uM{\dddxM}
\def\ddxm{\xm{1}}
\def\ddxM{\xM{1}}
\def\dxm{\xm{2}}
\def\dxM{\xM{2}}
\def\dym{\ym{2}}
\def\dyM{\yM{2}}
\def\ddym{\ym{1}}
\def\ddyM{\yM{1}}

\def\umM{(\um-\uM)}
%\def\umM{\ddot x_{\mbox{\tiny{mM}}}}
\def\Dp{(y_1^2 - 2y_2\um)}
\def\Dm{(y_1^2 - 2y_2\uM)}

\def\uu{\hat u_1}
\def\ud{\hat u_2}
\def\udu{(\ud-\uu)}
\def\uud{(\uu-\ud)}

\def\Dd{(y_1^2 - 2y_2\ud)}
\def\Du{(y_1^2 - 2y_2\uu)}


